Evolutionary Diversity Optimization and the Minimum Spanning Tree Problem

In the area of evolutionary computation the calculation of diverse sets of high-quality solutions to a given optimization problem has gained momentum in recent years under the term evolutionary diversity optimization. Theoretical insights into the working principles of baseline evolutionary algorithms for diversity optimization are still rare. In this paper we study the well-known Minimum Spanning Tree problem (MST) in the context of diversity optimization where population diversity is measured by the sum of pairwise edge overlaps. Theoretical results provide insights into the fitness landscape of the MST diversity optimization problem pointing out that even for a population of $\mu=2$ fitness plateaus (of constant length) can be reached, but nevertheless diverse sets can be calculated in polynomial time. We supplement our theoretical results with a series of experiments for the unconstrained and constraint case where all solutions need to fulfill a minimal quality threshold. Our results show that a simple $(\mu+1)$-EA can effectively compute a diversified population of spanning trees of high quality.

==> tables/uniform_weights.tex <==
\begin{table}[ht]
\caption{\label{tab:uniform_weights}Comparison in terms of diversity (\textbf{$D_o$}), the mean number of iterations (\textbf{mean}) until the algorithm terminated, the standard deviation of iterations (\textbf{std}) and results of Wilcoxon-Mann-Whitney tests (\textbf{stat}). The data is split by the sampling strategy (Uniform or Poisson). Here, $X^{+}$ means that the number of iterations is significantly better, i.e. lower, for the respective strategy. Lowest mean values per row are \colorbox{gray!20}{\textbf{highlighted}}.}
\renewcommand{\tabcolsep}{2pt}
\centering
\begin{scriptsize}
\begin{tabular}[t]{rrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{4}{c}{\textbf{Single (1)}} & \multicolumn{4}{c}{\textbf{Poisson (2)}} \\
\cmidrule(l{3pt}r{3pt}){3-6} \cmidrule(l{3pt}r{3pt}){7-10}
$n$ & $\mu$ & $D_o$ & \textbf{mean} & \textbf{std} & \textbf{stat} & $D_o$ & \textbf{mean} & \textbf{std} & \textbf{stat}\\
\midrule
 & 2 & 100.00 & 496.57 & 213.1 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{202.73}} & 71.07 & \textcolor{black}{$\text{1}^{+}$}\\

 & 3 & 100.00 & 1148.50 & 483.8 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{464.80}} & 230.95 & \textcolor{black}{$\text{1}^{+}$}\\

 & 10 & 100.00 & 7545.70 & 2143.8 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{3556.10}} & 1003.74 & \textcolor{black}{$\text{1}^{+}$}\\

\multirow{-4}{*}{\raggedleft\arraybackslash 50} & 20 & 100.00 & \cellcolor{gray!20}{\textbf{40974.07}} & 7748.7 & \textcolor{black}{$\text{2}^{+}$} & 99.99 & 45684.20 & 6732.28 & $\text{1}^{-}$\\
\cmidrule{1-10}
 & 2 & 100.00 & 1635.97 & 430.7 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{514.30}} & 186.10 & \textcolor{black}{$\text{1}^{+}$}\\

 & 3 & 100.00 & 2997.97 & 1112.8 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{1133.07}} & 326.23 & \textcolor{black}{$\text{1}^{+}$}\\

 & 10 & 100.00 & 16857.03 & 3883.4 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{7158.87}} & 1532.67 & \textcolor{black}{$\text{1}^{+}$}\\

 & 20 & 100.00 & 47340.73 & 12423.7 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{29357.97}} & 5591.27 & \textcolor{black}{$\text{1}^{+}$}\\

\multirow{-5}{*}{\raggedleft\arraybackslash 100} & 50 & 99.93 & 500000.00 & 0.0 & $\text{2}^{-}$ & 99.89 & 500000.00 & 0.00 & $\text{1}^{-}$\\
\cmidrule{1-10}
 & 2 & 100.00 & 4855.40 & 1186.0 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{1657.57}} & 635.46 & \textcolor{black}{$\text{1}^{+}$}\\

 & 3 & 100.00 & 9012.30 & 2736.5 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{2971.77}} & 852.22 & \textcolor{black}{$\text{1}^{+}$}\\

 & 10 & 100.00 & 40965.93 & 8380.8 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{16909.13}} & 4538.21 & \textcolor{black}{$\text{1}^{+}$}\\

 & 20 & 100.00 & 109356.77 & 18658.4 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{50028.87}} & 11589.15 & \textcolor{black}{$\text{1}^{+}$}\\

 & 50 & 100.00 & 468135.27 & 98711.2 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{384015.73}} & 85902.52 & \textcolor{black}{$\text{1}^{+}$}\\

\multirow{-6}{*}{\raggedleft\arraybackslash 200} & 100 & 99.98 & 4000000.00 & 0.0 & $\text{2}^{-}$ & 99.95 & 4000000.00 & 0.00 & $\text{1}^{-}$\\
\cmidrule{1-10}
 & 2 & 100.00 & 14387.47 & 3715.4 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{5446.33}} & 2206.11 & \textcolor{black}{$\text{1}^{+}$}\\

 & 3 & 100.00 & 27128.97 & 8431.9 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{8544.87}} & 2246.86 & \textcolor{black}{$\text{1}^{+}$}\\

 & 10 & 100.00 & 129626.07 & 21497.3 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{45131.17}} & 12767.99 & \textcolor{black}{$\text{1}^{+}$}\\

 & 20 & 100.00 & 297361.97 & 51641.4 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{120375.70}} & 35664.42 & \textcolor{black}{$\text{1}^{+}$}\\

 & 50 & 100.00 & 978074.13 & 142066.8 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{480851.63}} & 78763.77 & \textcolor{black}{$\text{1}^{+}$}\\

\multirow{-6}{*}{\raggedleft\arraybackslash 400} & 100 & 100.00 & 3574319.67 & 656421.4 & $\text{2}^{-}$ & 100.00 & \cellcolor{gray!20}{\textbf{2704053.33}} & 511598.25 & \textcolor{black}{$\text{1}^{+}$}\\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{table}
